Preservation of the Global Knowledge by Not-True Distillation in Federated Learning

In federated learning, a strong global model is collaboratively learned by aggregating clients' locally trained models. Although this precludes the need to access clients' data directly, the global model's convergence often suffers from data heterogeneity. This study starts from an analogy to continual learning and suggests that forgetting could be the bottleneck of federated learning. We observe that the global model forgets the knowledge from previous rounds, and the local training induces forgetting the knowledge outside of the local distribution. Based on our findings, we hypothesize that tackling down forgetting will relieve the data heterogeneity problem. To this end, we propose a novel and effective algorithm, Federated Not-True Distillation (FedNTD), which preserves the global perspective on locally available data only for the not-true classes. In the experiments, FedNTD shows state-of-the-art performance on various setups without compromising data privacy or incurring additional communication costs.

==> 03-approach_backup.tex <==
\vspace{-2pt}
\section{FedNTD: Federated Not-True Distillation}
\vspace{-6pt}

\begin{wrapfigure}{r}{0.5\textwidth}
    \vspace{-18pt}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/ntd_concept.png}
    \vspace{-15pt}
\caption{\small An overview of Not-True Distillation.The true class (\textit{Class 3}) logits is ignored in the softmax.}
\label{fig:ntd}
\end{wrapfigure}

In this section, we propose Federated Not-True Distillation (FedNTD) and its key features. The core idea of FedNTD is to preserve the global view only for the not-true classes. More specifically, FedNTD conducts local-side distillation by the linearly combined loss function $\mathcal{L}$ between the cross-entropy loss $\mathcal{L}_{\textup{CE}}$ and the not-true distillation loss $\mathcal{L}_{\textup{NTD}}$:
\begin{equation}
\mathcal{L} = \mathcal{L}_{\textup{CE}}(q^{l}, \; \mathds{1}_y) + \beta \cdot \mathcal{L}_{\textup{NTD}}({\tilde{q}_{\tau}^{l}}, \; {\tilde{q}_{\tau}^{g}}).
\label{eq:fedntd}
\end{equation}

\vspace{-4pt}
Here, the hyperparameter $\beta$ stands for the strength of knowledge preservation on the out-local distribution. Then, the not-true distillation loss $\mathcal{L}_{\textup{NTD}}$ is defined as the KL-Divergence loss between the not-true softmax prediction vector ${\tilde{q}_{\tau}}^{l}$ and ${\tilde{q}_{\tau}^{g}}$ as follows:
%
\begin{equation}
\small
{\mathcal{L}}_{\text{NTD}}({\tilde{q}_{\tau}^{l}},{\tilde{q}_{\tau}^{g}})=-\!\sum_{c=1\,, \underline{\mathbf{c \neq y}}}^{C}{\tilde{q}_{\tau}^{g}}(c)\log\left[\frac{{\tilde{q}_{\tau}^{l}}(c)}{{\tilde{q}_{\tau}^{g}}(c)}\right]\,,
%
\:\: \text{where}\:\:
%
\begin{cases}
\normalsize
{\tilde{q}_{\tau}^{l}}(c) =\frac{ \exp{({z}_{c}^{l}/\tau)}}{\sum_{\underline{\mathbf{\tilde{c} \neq y}}}^{C}\exp{({z}_{\tilde{c}}^{l}/\tau)}}
\vspace{8pt}
\\
{\tilde{q}_{\tau}^{g}}(c) =\frac{ \exp{({z}_{c}^{g}/\tau)}}{\sum_{\underline{\mathbf{\tilde{c} \neq y}}}^{C}\exp{({z}_{\tilde{c}}^{g}/\tau)}}
\end{cases} \!\!(\forall c \neq y).
\end{equation}
%
which take softmax with temperature $\tau$ only for the not-true class logits. \autoref{fig:ntd} illustrates how the not-true distillation works given a sample $x$. Note that ignoring the true-class logits makes gradient signal of $\mathcal{L}_{\textup{NTD}}$ to the true-class as $0$. The detailed algorithm is provided in \autoref{appendix_algorithm}.

We now explain how learning to minimize $\mathcal{L}_{\textup{NTD}}$ preserves global knowledge on out-local distribution $\tilde{p}(\mathcal{D})$. Since it is well-known that KL-Divergence loss on the softmax outputs acts as matching their logits vectors to close their distance \citep{kd_mse, kd_survey, understanding_kd}, We start from a Mean-Squared Error (MSE) loss on the logits to simplify the discussion. Although not rigorous, this gives enough intuition to understand the effect of not-true distillation. An experimental validation is provided in \autoref{appendix_prop2_mse}.

Suppose there are $N$ number of data points in the local dataset $\mathcal{D}$. The accumulated MSE loss $\mathcal{L}_{\textup{MSE}}$ between $z_i^{c}$, the class $c$ logits of data $x_i$, and its reference logits $z_{i,\mathrm{ref}}^{c}$ to be matched for is:
\vspace{-2.5pt}
\begin{equation}
\small
\mathcal{L}_{\textup{MSE}}=\frac{1}{N\mathcal{C}}\sum_{i=1}^{N}\sum_{c=1}^{\mathcal{C}} (z_i^{c} - z_{i,\mathrm{ref}}^{c})^2\,.
\end{equation}

By splitting the the square term for the \textit{true} and \textit{not-true} classes, the term becomes:
%
\vspace{-2pt}
\begin{equation}
\small
\mathcal{L}_{\textup{MSE}}^{\textup{true}}=\frac{1}{N}\sum_{i=1}^{N}\sum_{c= y_i}^{\mathcal{C}} (z_i^{c} - z_{i,\mathrm{ref}}^{c})^2\,,
%
\qquad
%
\mathcal{L}_{\textup{MSE}}^{\textup{not-true}}=\frac{1}{N(\mathcal{C}-1)}\sum_{i=1}^{N}\sum_{c'\neq y_i}^{\mathcal{C}} (z_i^{c'} - z_{i,\mathrm{ref}}^{c'})^2\,.
\label{eq:nt_mse}
\end{equation}

\vspace{1pt}
\begin{proposition}
Consider the in-local distribution $p(\mathcal{D}) = [p_1 \dots p_{\mathcal{C}}]$ such that $p_c = \frac{|\mathcal{S}_c|}{N}$ and its  out-local distribution $\tilde{p}(\mathcal{D}) = [\tilde{p}_1, \dots \tilde{p}_{\mathcal{C}}]$, where $\mathcal{S}_c$ is the set of indices satisfying $y_i=c$. Then the $\mathcal{L}_{\textup{MSE}}^{\textup{true}}$ and $\mathcal{L}_{\textup{MSE}}^{\textup{not-true}}$ each are equivalent to the weighted sum on $p(\mathcal{D})$ and $\tilde{p}(\mathcal{D})$ as
\begin{equation}
\small
\mathcal{L}_{\textup{MSE}}^{\textup{true}}= \sum_{c=1}^\mathcal{C} \: \boldsymbol{p_c}  \: \bigg[ \frac{\sum_{i\in\mathcal{S}_{c}}(z_i^{c} - z_{i,\mathrm{ref}}^{c})^2}{|\mathcal{S}_{c}|} \bigg],
%
\qquad
%
\mathcal{L}_{\textup{MSE}}^{\textup{not-true}}= \sum_{c=1}^\mathcal{C} \: \boldsymbol{\tilde{p}_c} \: \bigg[\frac{\sum_{i\notin\mathcal{S}_{c}}(z_i^{c} - z_{i,\mathrm{ref}}^{c})^2}{\sum_{c'\neq c} |\mathcal{S}_{c'}|} \bigg].
\end{equation}
where the term in $[\cdot]$ represents the normalized logits MSE for each class.
\label{prop1:ntd}
\end{proposition}
%
\vspace{-2pt}
With a minor amount of calculation from \autoref{eq:nt_mse}, we derive the above proposition. The derivation is provided in \autoref{proof_proposition2}. The proposition suggests that matching the true-class and the not-true class logits collapses to the loss on the in-local distribution $p(\mathcal{D})$ and the out-local distribution $\tilde{p}(\mathcal{D})$. 

In the loss function of our FedNTD (\autoref{eq:fedntd}), we attain the new knowledge on the in-local distribution by following the true-class signals from the labeled data in local datasets using the $\mathcal{L}_{\textup{CE}}$. In the meanwhile, we preserve the previous knowledge on the out-local distribution by following the global model's perspective, corresponding to the not-true class signals, using the $\mathcal{L}_{\textup{NTD}}$. Here, the hyperparameter $\beta$ controls the trade-off between learning on the new knowledge and preserving previous knowledge. This resembles to \textit{stability-plasticity dilemma} \citep{stability-plasticity} in continual learning, where the learning methods must balance retaining knowledge from previous tasks while learning new knowledge for the current task \citep{class_incremental_survey}.
